On the Inconsistency of Kernel Ridgeless Regression in Fixed Dimensions

``Benign overfitting'', the ability of certain algorithms to interpolate noisy training data and yet perform well out-of-sample, has been a topic of considerable recent interest. We show, using a fixed design setup, that an important class of predictors, kernel machines with translation-invariant kernels, does not exhibit benign overfitting in fixed dimensions. In particular, the estimated predictor does not converge to the ground truth with increasing sample size, for any non-zero regression function and any (even adaptive) bandwidth selection. To prove these results, we give exact expressions for the generalization error, and its decomposition in terms of an approximation error and an estimation error that elicits a trade-off based on the selection of the kernel bandwidth. Our results apply to commonly used translation-invariant kernels such as Gaussian, Laplace, and Cauchy.

==> no_arxiv/old/highd_app_old.tex <==
\section{Results for dimension greater than 1}
\label{app:highd}

\subsection{Preliminaries}

$\Omega=(-\pi,\pi]^d$ and Kernel $k(x_1,x_2) = g(M_1((x_1-x_2)_1\mod\Omega), ..., M_d((x_1-x_2)_d\mod\Omega)) = g(\{M_i((\x_1-\x_2)_i\mod\Omega)\}_i)$. We will suppose $M_i = M$ for all $i \in [d]$. 

\begin{align}
    g(\{M_i((\x_1-\x_2)_i\mod\Omega)\}_i) &= \sum_{\k \in\Integer^d} G[\k]\exp(j\k \cdot (\x_1-\x_2))\\
    G[\k] &= \frac{1}{(2\pi)^d} \int_\Omega g(\{M_i(\x_i\mod\Omega)\}_i) \exp(-j \k \cdot \x)\dif \x
\end{align}

\begin{definition}
Let $X[\k]=X_{\k}=\mathcal{FS}\{x\}[\k]$ be the $\k$-th Fourier series coefficient of $x:\Omega \rightarrow \Real$, where $\k\in\Integer^d$.
\end{definition}

\subsection{Fourier analysis}

\begin{definition}
Let $\phi_k(x) = \frac{1}{\sqrt{2\pi}} e^{jkx}$ for $k\in\Integer$. In higher dimensions, for $\k \in \Integer^d$, $\phi_{\k}(\x) = \prod_{i=0}^{d-1} \phi_{k_i}(x_i)$.
\end{definition}

\begin{definition}[Circular Convolution]
For $f,g:\Omega\rightarrow\Real$ we define the operator
\begin{align}
    (f\circconv g)(t) = \frac{1}{2\pi} \int_{\Omega}f(\tau)g(t-\tau \mod \Omega)\dif\tau
\end{align}
\end{definition}

For a fixed $N\in\Natural,$ for $\ell\in[N]^d$, let $G_{\ell} \in \ell^2$ be the subsequence with entries 
\begin{align}
G_{\ell}[\m] = G[\m N + \ell],\qquad \forall\,\m\in\Integer^d   
\end{align}

As the target function is defined on the unit torus, it admits a Fourier series, 
\begin{align}\label{eq:target_fn_highd}
f^* = \sum_{\k \in \mathbb{Z}^d} V[\k] \phi_{\k}    
\end{align}
Further, for a fixed $N\in\Natural,$ and for $\ell\in[N]^d$, let $V_{\ell} \in \ell^2$ be the subsequence with entries 
\begin{align}
V_{\ell}[\m] = V[\m N + \ell],\qquad \forall\,\m\in\Integer^d   
\end{align}


\subsubsection{Assumptions}

\begin{definition}
Let $S_Q$ be the set of $\k \in \Integer^d$ such that $|k_i| \leq Q$ for all $i \in [d]$. Let $S^c_Q$ be the complement of this set (in the universe $\Integer^d$). 
\end{definition}

\begin{assumption}[Scale]
\label{ass:scale}
$\displaystyle\sum_{\k \in \mathbb{Z}^d} |G[\k]| < \infty$.
\end{assumption}

\begin{assumption}[Tail of spectrum]
\label{ass:tail}
For all $k \in \Integer_{\geq 0}$, there exists a constant $C_1 > 0$ such that,
\begin{align}\label{eq:tail_assumption}
    |G[M^\prime k + i]| \leq \frac{C_1 |G[i]|}{1 + k^2}
\end{align}
holds for all $M'\geq M$ and for all $i \leq M'$, except $o_{M'}(M')$ many.
\end{assumption}

\begin{assumption}[Head of spectrum]
\label{ass:head}
There exist constants $C_2, C_3\in\Real_+$ and $i^*\in\Integer_{\geq 0}$ such that for $M\geq C_2$, we have that for all $M'\leq M$, $|G[i^*]| \leq C_3 |G[i^*+M']|$  and $\abs{G_0[i^*]}>0$.
\end{assumption}

\subsection{Noisy estimation error}

Let $\varepsilon(t) = \inner{\K\inv\xivec,K(X_N,t)}_n$ for $t \in \Omega$. This is a periodic function in $t$ with period $2\pi$ in each coordinate. Therefore, there exists a set of Fourier coefficients $E_{\k}$ for $\k \in \mathbb{Z}^d$ such that:
\begin{align}
    \varepsilon(t) = \sum_{\k\in\Integer^d} E_{\k} e^{-j 2\pi \k \cdot t}
\end{align}

\begin{lemma}
\label{lemma:coeff_inspan_highd}
\begin{align}
    E_{\k} = (\Kmat\inv \xivec) \cdot (e^{-j \k \cdot \x_{\p}})_{n} G[\k]
\end{align}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:coeff_inspan_highd}]
\begin{align}
    \inner{\Kmat\inv\xivec,K(X_N,t)}_N &= \sum_{\p \in [N]^d} (\Kmat\inv\xivec)_{\p} g(t - \x_{\p})\\
    &= \sum_{n \in [N]^d} \int_\Omega (\Kmat\inv\xivec)_{\p} g(t - \x_{\p}) (\Kmat\inv\xivec)_{\p} g({\x}^\prime - t) \delta(x^\prime - t_{\p}) \dif{\x}^\prime \\
    &= \int_\Omega \sum_{n \in [N]^d} g({\x}^\prime - t) (\Kmat\inv\xivec)_{\p} \delta({\x}^\prime - t_{\p}) \dif {\x}^\prime \\
    &= \rbrac{ \sum_{\p} (\Kmat\inv\xivec)_{\p} \delta_{\x_{\p}} \circconv^d g}(t) 
\end{align}

Applying Lemma \ref{lemma:highd_conv_omega}, using that $\FS{\x+\y}[\k] = \FS{\x}[\k] + \FS{\y}[\k]$, and where $E_{\k}$ is the $\k$-th Fourier series coefficient of $\varepsilon=\widehat{f} - f^*$, we see that:
\begin{align}
    E_{\k} &= (2\pi)^d \FS{\sum_{\p} (\Kmat\inv \xivec)_{\p} \delta_{x_{\p}}}[\k] \cdot G[\k] \\
    &= (\Kmat\inv \xivec) \cdot (e^{-j \k \cdot \x_{\p}})_n G[\k]
\end{align}
where we have used $\FS{\delta_{\x_{\p}}}[\k]= \frac{1}{(2\pi)^d} e^{-j\k \cdot \x_{\p}}$ and $\FS{a \delta_{\x_{\p}}}[\k] = a \FS{\delta_{\x_{\p}}}[\k]$ for $a \in \mathbb{R}$. 

%$\FS{\sum_{n}\delta_{x_n}}[k]=\sum_{n}\delta_{\frac{2\pi x_n}{N}}[k]$. 

Using these formula and that we sample $x_{\p} = (\frac{2\pi p_0}{N},...,\frac{2\pi p_{d-1}}{N})$ for $\p = (p_1,...,p_d) \in [N]^d$, we derive the main lemma.
\end{proof}

\begin{lemma}
\label{lemma:noise_dft_d}
Let $\xivec \in \mathbb{R}^{N^d}$ be a vector of i.i.d. random variables with variance $\sigma^2$ and mean $0$. Let $\omega \in \mathbb{R}^d$.
\begin{align}
    \Exp_{\xivec} |(\Kmat\inv \xivec) \cdot (e^{-j \omega \cdot \x_{\p}})_n|^2 = \sigma^2 \trace \left( \Kmat^{-2} (e^{j\omega \cdot \p})_n \herm (e^{-j\omega \cdot \p})_{n}) \right)
\end{align}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:noise_dft_d}]
\begin{align*}
    \Exp_{\xivec} \left( \sum_{\p,{\p}^\prime \in [N]^d} \Kmat\inv_{\p,{\p}^\prime} \xi_{\p^\prime} e^{-j \omega \cdot \p} \right) \left( \sum_{\p,\p^\prime \in [N]^d} \Kmat\inv_{\p,\p^\prime} \xi_{\p^\prime} e^{j \omega \cdot \p} \right)
    &= \sigma^2 \sum_{\p^\prime \in [N]^d} \sum_{\p,\m \in [N]^d} \Kmat^{-1}_{\p,\p^\prime} \Kmat^{-1}_{\p^\prime,\m} e^{-j\omega \cdot (\p-\m)} \\ 
    &= \sigma^2 \sum_{\p,\m} \Kmat^{-2}_{\p,\m} e^{-j \omega \cdot (\p-\m)} \\
    &= \sigma^2 \trace \left( \Kmat^{-2} (e^{j\omega \cdot \p})_n \herm (e^{-j\omega \cdot \p})_n \right)
\end{align*}
\end{proof}

\begin{lemma} 
\label{lem:estimation_error_highd}
For $d$ dimensions, the noisy estimation error satisfies:
\begin{align}
    \text{Noisy Estimation Error} = \sigma^2 \sum_{\p \in [N]^d} \frac{\sum_{\m \in \mathbb{Z}^d} |G^{M}[\m N +\p]|^2}{\left|\sum_{\k \in \mathbb{Z}^d} G^{M}[\k N +\p]\right|^2}
\end{align}
\end{lemma}
\begin{proof}
By Theorem \ref{thm:parseval_continuous} in the first line, Lemma \ref{lemma:coeff_inspan} in the third, and Lemma \ref{lemma:noise_dft_d} in the last,
\begin{align}
    \Exp \sbrac{ \frac{1}{(2\pi)^d} \int_\Omega |\varepsilon(\t)|^2 \dif \t } &= \sum_{\k\in\Integer^d} \Exp |E_{\k}|^2 \\
    &= \sum_{\p \in [N]^d} \sum_{\m \in \Integer^d} \Exp |E_{\m N + \p}|^2 \\
    &= \sum_{\p \in [N]^d} \sum_{\m \in \Integer^d} \left|G[\m N + \p]\right|^2 \Exp \left|(\Kmat\inv \xivec) \cdot (e^{-j \k \cdot \x_{\p}})_n \right|^2 \\
    &= \sigma^2 \sum_{\p \in [N]^d} \sum_{\m \in \Integer^d} \left|G[\m N+\p]\right|^2  \trace \left( \Kmat^{-2} (e^{j\omega \cdot \p})_n \herm (e^{-j\omega \cdot \p})_n \right) \\
    &= \sigma^2 \sum_{\p \in [N]^d} \sum_{\m \in \Integer^d} \frac{|G[\m N+\p]|^2}{\left|\sum_{\k \in \mathbb{Z}^d} G[\k N + \p] \right|^2}
\end{align}
The last line follows by evaluating the trace.
\end{proof}



\subsection{Noise-free estimation and approximation errors}

\begin{lemma}
\label{lemma:phi_mod_highd}
For $N$ evenly sampled points on the unit torus,
\begin{align*}
    {\phi_{\k}(x_n) = \phi_{\k \mod N}(x_n) = \phi_{k_1 \mod N}(x_{n,1}) \times \cdots \times \phi_{k_d \mod N}(x_{n,d})}
\end{align*} for $n \in [N]^d$, where $\k \mod N$, $\k\in\Integer^d$ acts component-wise. 
\end{lemma}

% \begin{definition}
% The tensored DFT matrix is the $d$-fold Kronecker product of the 2-dimensional DFT matrix $U$ with itself.
% \begin{align}
%     U^d = \underbrace{U \otimes \cdots \otimes U}_{d}
% \end{align}
% We will write the d-dimensional DFT vector $\u_{\ell}^d$ (of length $N^d$) as the $\ell$-th column of this matrix.
% \end{definition}

% \begin{definition}
% In high dimension $d$, the kernel matrix is the defined in the following manner. For the 1-d kernel $k$, let the $1$-d kernel matrix be:
% \[
% K^{(1)} = \begin{bmatrix}
%     k(x_1 - x_1)& \cdots & k(x_N - x_1) \\
%     k(x_1 - x_2) & \cdots & k(x_N - x_2)  \\
%     \vert & \cdots & \vert \\
%     k(x_1 - x_N)& \cdots & k(x_N - x_N)
% \end{bmatrix}
% \]
% Then, the multidimensional kernel matrix $K^{(d)}$ is defined as:
% \begin{align}
%     K^{(d)} = \underbrace{K^{(1)} \otimes \cdots \otimes K^{(1)}}_{d}
% \end{align}
% %Further, let $K^{(1)}_{ij} = K^{(1)} k(x_i - x_j)$. Then, the multi-dimensional kernel matrix $\in \mathbb{R}^{N^d}$ is defined recursively,
% %\[
% %K^{(d)} = K^{(d-1)} \otimes K^{(1)} = %\begin{bmatrix}
% %    K^{(d-1)}_{11} & \cdots & K^{(d-1)}_{1N} \\
% %    K^{(d-1)}_{21} & \cdots & K^{(d-1)}_{2N}  \\
% %    \vdots & \cdots & \vdots \\
%  %   K^{(d-1)}_{N1} & \cdots & K^{(d-1)}_{NN}
% %\end{bmatrix}
% %\]
% \end{definition}

% \begin{fact}
% The eigenvectors of $K^{(d)}$ are tensor products of the eigenvectors of $K^{(1)}$, and their eigenvalues are the product of the eigenvalues of the $1$-d kernel matrix.
% \end{fact}

% \begin{fact}
% The eigenfunctions of the empirical covariance operator in $d$-dimensions are products over $\psi_k$ - the eigenfunctions of the empirical covariance operator in $1$-dimensions.
% \end{fact}

For a function $f^*\in L^2,$ define,
\begin{align}c_{\ell,f^*} = \frac{\sum_{\m \in \Integer^d} G[\m N + \ell] v_{\m N + \ell}}{\sum_{\m \in \Integer^d} (G[\m N + \ell])^2}, \qquad \ell\in[N]^d
\end{align}

\begin{lemma}
\label{lemma:orthogonal_comp_highd}
Let $f^* = \sum_{\k \in \Integer^d} v_{\k} \phi_{\k}$ for $\v_{k} \in \mathbb{R}$. We have, 
\begin{align}
    P_{\X}f^* = \frac{1}{(2\pi)^{d/2}} c_{\ell,f^*} \sum_{\m \in \Integer^d} G[\m N + \ell] e^{j(\m N + \ell)\cdot x} 
\end{align}
Further, \begin{align}
\|f^*-P_{\X}f^*\|^2_{L^2} = \sum_{\k \in \Integer^d} v^2_{\k} - \sum_{\ell \in [N]^d} \frac{\rbrac{\sum_{\m \in \Integer^d} G[\m N + \ell] v_{\m N + \ell}}^2}{\sum_{\m \in \Integer^d} (G[\m N + \ell])^2}.
\end{align}
\end{lemma}
\begin{proof}
Here we drop the subscript $L^2$ (all norms, inner products are $L^2$ unless specified otherwise). Let $\psi_{\ell}$ be a basis function for $\ell \in [N]^d$. As in $2$-d, because the span of the representers has $\frac{\psi_\ell}{\|\psi_\ell\|}$ as an orthonormal basis, we have \begin{align*}
    P_{\X}f^* &= \sum_{\ell \in [N]^d} \inner{f^*, \frac{\psi_\ell}{\|\psi_\ell\|}} \frac{\psi_\ell}{\|\psi_\ell\|}\\
    \norm{P_{\X}f^*}^2 &= \sum_{\ell \in [N]^d} \inner{f^*, \frac{\psi_\ell}{\|\psi_\ell\|}}^2
\end{align*} 

Let $\lambda_{\ell} = \prod_{i=1}^d \lambda_{\ell_i}$ Then,
\begin{align}
    \inner{f^*,\psi_{\ell}} = \sqrt{\frac{(2\pi N)^d}{\lambda_{\ell}}} \sum_{\m \in \Integer^d} G[\m N + \ell] v_{\m N + \ell} 
\end{align}
Recall from Lemma \ref{lem:psi_orthonormal_highd} that
\begin{align}
    \|\psi_{\ell}\|_{L^2} = \sqrt{\frac{(2\pi N)^d}{\lambda_\ell} \sum_{\m \in \Integer^d} \rbrac{G[\m N + \ell]}^2},\qquad \ell\in[N]^d. 
\end{align}
Then, for $\ell \in [N]^d$,
\begin{align}
    \inner{f^*, \frac{\psi_\ell}{\|\psi_\ell\|}} \frac{\psi_\ell}{\|\psi_\ell\|} &= \frac{1}{(2\pi)^{d/2}} \frac{\rbrac{\sum_{\m \in \Integer^d} G[\m N + \ell] e^{j(\m N + \ell)\cdot x} } \rbrac{\sum_{\m \in \Integer^d} G[\m N + \ell] v_{\m N + \ell}}}{\sum_{\m \in \Integer^d} (G[\m N + \ell])^2} \\
    &= \frac{1}{(2\pi)^{d/2}} c_{\ell,f^*} \sum_{\m \in \Integer^d} G[\m N + \ell] e^{j(\m N + \ell)\cdot x} 
\end{align}
The first claim follows.

For the second claim, we see that:
\begin{align}
    \norm{P_{\X}f^*}^2 &= \sum_{\ell \in [N]^d} \frac{(2\pi N)^d}{\lambda_{\ell}} \frac{1}{\|\psi_{\ell}\|^2} \rbrac{\sum_{\m \in \Integer^d} G[\m N + \ell] v_{\m N + \ell}}^2 \\ 
    &= \sum_{\ell \in [N]^d} \frac{\rbrac{\sum_{\m \in \Integer^d} G[\m N + \ell] v_{\m N + \ell}}^2}{\sum_{\m \in \Integer^d} (G[\m N + \ell])^2}
\end{align}
As $P_{\X}$ is the $L^2$ projection onto the span of the representers, the main lemma follows by the Pythagorean theorem.
\end{proof}

\begin{lemma}
Let $(f^* - P_{\X}f^*)_n$ be the vector of $f^* - P_{\X}f^*$ evaluated on the data with the same ordering as the kernel matrix $\Kmat$. Then,
\begin{align}
    \abs{ \K\inv(f^* - P_{\X}f^*)_n \cdot {\u}_{\k}}^2
    &= \frac{1}{(2\pi)^d} \rbrac{\frac{\|V_{\k}\|_1}{\|G_{\k}\|_1} - \frac{G_{\k} \cdot V_{\k} }{\|G_{\k}\|^2_2}}^2
\end{align}
% \begin{align}
%     \abs{ \K\inv(f^* - P_{\X}f^*)_n \cdot {\u}_{\k}}^2
%     &= \frac{1}{(2\pi)^d} \rbrac{\frac{\sum_{\m \in \Integer^d} v_{\m M + \k}}{\sum_{\m \in \Integer^d} G[\m N + \k]} - \frac{\sum_{\m \in \Integer^d} G[\m N + \k] v_{\m N + \k}}{\sum_{\m \in \Integer^d} (G[\m N + \k])^2}}^2
% \end{align}
\end{lemma}
\begin{proof}
Let $\beta_{\k,f^*} = \sum_{\m \in \Integer^d} V[\m N + \k]$ for $\k \in [N]^d$.

By lemma \ref{lem:psi_orthonormal_highd}, lemma \ref{lemma:orthogonal_comp_highd}, and lemma \ref{lemma:phi_mod_highd}, we can write $Pf^*$ on a datapoint $x_{\p}$ with $\p \in [N]^d$ as
\begin{align}
    P_{\X}f^*(x_{\p}) = \frac{1}{(2\pi)^{d/2}} \sum_{\ell \in [N]^d} c_{\ell,f^*} \beta_{\ell,f^*} e^{j\ell \cdot x_{\p}} 
\end{align}
Then, where $\tilde{\beta} = ((\beta_{\ell} - c_{\ell,f^*} \|G_{\ell}\|_1)_{\ell \in [N]^d})\tran$, $\Lambda = (\lambda_{\ell})_{\ell}$, and $U$ is the $d$-dimensional DFT matrix (a $d$-fold Kronecker product of the $1$-d DFT matrix).
\begin{align}
    \Kmat\inv(f^* - Pf^*)_n \cdot u_k &= \frac{1}{(2\pi)^{d/2}} \rbrac{\Kmat\inv \rbrac{\sum_{\ell \in [N]^d} (\beta_{\ell,f^*} - c_{\ell,f^*} \|G_{\ell}\|_1) e^{j \ell \cdot x_{\p}}}_n }\tran v_k \\
    &= \frac{1}{(2\pi)^{d/2}} \rbrac{\Kmat\inv U \tilde{\beta}}\tran v_k \\
    &= \frac{1}{(2\pi)^{d/2}} \rbrac{U \Lambda^{-1} \tilde{\beta}}\tran v_k \\
    &= \frac{1}{(2\pi)^{d/2}} \tilde{\beta}^T \Lambda^{-1} U u_k \\
    &= \frac{1}{(2\pi)^{d/2}} \tilde{\beta}_k \lambda_k^{-1} \\
    &= \frac{1}{(2\pi)^{d/2}} \frac{\beta_{k} - c_{k,f} \|G_{k}\|_1}{\sum_{m \in \Integer} G[\m N + \k]} \\
    &= \frac{1}{(2\pi)^{d/2}} \frac{\sum_{\m \in \Integer^d} v_{\m M + \k} - \frac{\rbrac{\sum_{\m \in \Integer^d} G[\m N + \k]} \rbrac{\sum_{\m \in \Integer^d} G[\m N + \k] v_{\m N + \k}}} {\sum_{\m \in \Integer^d} (G[\m N + \k])^2}}{\sum_{\m \in \Integer^d} G[\m N + \k]} \\
    &= \frac{1}{(2\pi)^{d/2}} \rbrac{\frac{\sum_{\m \in \Integer^d} v_{\m M + \k}}{\sum_{\m \in \Integer^d} G[\m N + \k]} - \frac{\sum_{\m \in \Integer^d} G[\m N + \k] v_{\m N + \k}}{\sum_{\m \in \Integer^d} (G[\m N + \k])^2}}
\end{align}
\end{proof}

\begin{lemma}[MSE Expression ($d>1$)]
\label{lemma:MSE_highd}
\begin{align}
    &\Exp_\xi{\sbrac{\text{MSE}}} = \frac{1}{(2\pi)^d} \rbrac{\|V\|^2_2 - \sum_{\p \in [N]^d} \frac{\rbrac{G_{\p} \cdot V_{\p}}^2}{\|G_{\p}\|^2_2}} \\
    &+ \frac{1}{(2\pi)^d N^d} \sum_{\p \in [N]^d} \rbrac{\frac{\|V_{\p}\|_1}{\|G_{\p}\|_1} - \frac{G_{\p} \cdot V_{\p}}{\|G_{\p}\|^2_2} }^2 \|G_{\p}\|^2_2 \\
    & + \frac{\sigma^2}{N^d} \sum_{\p \in [N]^d}  \frac{\|G_{\p}\|^2_2}{\|G_{\p}\|^2_1}
\end{align}
\end{lemma}


\subsection{Inconsistency for all Bandwidths (\texorpdfstring{$d>1$}{d>1})}


\begin{theorem}
\label{theorem:inconsistent_all_band_highd}
There exists a linear subspace of functions in $\mathcal{H}_0$ (the base RKHS) for which kernel interpolation will be inconsistent for any bandwidth.
\end{theorem}

\begin{proof}[Proof of \Cref{theorem:inconsistent_all_band_highd}]

The proof mimics that of the $1$-d case. We consider two cases. Where $M \leq N$, and $M > N$. 
\end{proof}
\subsection{Deferred results}

\subsubsection{Fourier analysis}
\begin{theorem}[Parseval's theorem in high dimensions]
\label{thm:highd_parseval_continuous}
For a $2\pi$-periodic signal $f(\t)$ in $d$ dimensions with Fourier series coefficients $c_{\k}$ for $k \in \Integer^d$, we have
\begin{align}
    \sum_{\k \in \Integer^d} |c_{\k}|^2 = \frac{1}{(2\pi)^d} \int_\Omega |f(\t)|^2 \dif \t
\end{align}
\end{theorem}

\begin{lemma}[Convolution is multiplication in high-$d$ Fourier domain]
\label{lemma:highd_conv_omega}
    Suppose $2\pi$-perioidic signals $x,y: \Omega \rightarrow \Real$ have Fourier series coefficients $X[\k],Y[\k]$ respectively for $\k \in \Integer^d$. Then, 
    \begin{align}
        \mathcal{FS}\{x \circconv^d y\}[\k] = (2\pi)^d X[\k] Y[\k] 
    \end{align}
\end{lemma}
\begin{proof} 
It suffices to show that $(x\circconv^d y)(t)=\sum_{\k \in\Integer^d}X_{\k} Y_{\k} \exp(j\k \cdot t)$. Now consider,
\begin{align}
    x(t) &= \sum_{\k \in\Integer^d} X_{\k} \exp(j\k \cdot t)\qquad
    y(t) = \sum_{\k \in\Integer^d} Y_{\k} \exp(j\k \cdot t)\\
    (x\circconv^d y)(t) &= \int_\Omega x(\tau) y(t-\tau \mod \Omega)\dif\tau\\
    &= \int_\Omega \rbrac{\sum_{\k \in\Integer^d} X_{\k} \exp(j \k \cdot \tau) }
    \rbrac{\sum_{\k^\prime \in\Integer^d} Y_{\k^\prime} \exp(j\k^\prime \cdot (t-\tau \mod \Omega))}\dif\tau\\
    &=\sum_{\k,\k^\prime\in\Integer}  X_{\k} Y_{\k^\prime} \int_\Omega    \exp(j\k \cdot \tau)  \exp(j\k^\prime \cdot (t-\tau \mod \Omega))\dif\tau\qquad\{t-\tau\longleftarrow u\}\\
    &=\sum_{\k,\k^\prime\in\Integer^d}  X_{\k} Y_{\k^\prime}\int_\Omega\exp(j\k \cdot (t-u)+j\k^\prime \cdot (u \mod \Omega))\dif u\\
    &=\sum_{\k,\k^\prime\in\Integer^d} X_{\k} Y_{\k}\exp(j\k \cdot t)\mathbf{1}_{\{\k=\k^\prime\}}\cdot (2\pi)^d
    =\sum_{\k \in\Integer^d}X_{\k} Y_{\k} \exp(j\k \cdot t)\cdot (2\pi)^d
\end{align}
which concludes the proof.
\end{proof}

\subsubsection{Approximation error lemmas}

\begin{lemma}[Eigenvectors of $\Kmat$ ($d > 1$)]\label{lem:eigenvectors_of_Kmat_highd}
The eigenvectors for $\Kmat$ are $\bar{u}_{\ell} = \{e^{-j \ell \cdot \x_{\p}}\}_{\p}$ for $\ell \in [N]^d$ with eigenvalues 
\begin{align}
N^d \lambda_\ell = N^d \sum_{\m \in \Integer^d} G[\m N + \ell].    
\end{align}
\end{lemma}

\begin{proof}[Proof of \Cref{lem:eigenvectors_of_Kmat_highd}]
\begin{subequations}
Let $i \in [N]^d$
\begin{align}
    (\Kmat v_{\ell})_{i} = \sum_{\p \in [N]^d} \Kmat_{i,\p} v_{\ell \p} &= \sum_{\p} \sum_{\m \in \Integer^d} G[\m] e^{j \frac{2\pi \m \cdot (i - \p)}{N}} e^{\frac{j 2\pi \p \cdot \ell }{N}} \\
    &= \sum_{\m \in \Integer} G[\m] e^{j \frac{2\pi \m \cdot i}{N}} \sum_{\p \in [N]^d}  e^{j \frac{2\pi (\ell-\m)\cdot \p}{N}} \\
    &= N^d \sum_{\m \in \Integer} G[\m N + \ell] e^{j \frac{2\pi (\m N + \ell) \cdot i}{N}} \\
    &= e^{j \frac{2\pi \ell \cdot i}{N}} N^d \sum_{m \in \Integer} G[mN + \ell] e^{j \frac{2\pi N \m \cdot i}{N}} \\
    &= e^{j \frac{2\pi \ell \cdot i}{N}} N^d \sum_{m \in \Integer} G[\m N + \ell] \\
    &= e^{j \frac{2\pi \ell \cdot i}{N}} N^d \lambda_\ell
\end{align}
\end{subequations}
\end{proof}

\begin{lemma}[Eigenfunctions of $\Kcov$ ($d > 1$)]\label{lem:eigenfunctions_of_Kcov_highd}
The eigenfunctions for the empirical kernel transform $\Kcov$ are,
\begin{align}
    \psi_\ell(x) &= \sqrt{\frac{N^d}{\lambda_\ell}} \sum_{\m \in \Integer} G[\m N + \ell] e^{j (\m N + \ell) \cdot x},\qquad \ell\in[N]^d.
\end{align}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:eigenfunctions_of_Kcov_highd}]
As in the $1$-d case, by Lemma \ref{lemma:eigvectors_covariance}, we have
\begin{align}
    \psi_{\ell}(x) &= \inner{\frac{(e^{-j \ell \cdot \x_{\p}})_n}{\sqrt{N^d \lambda_{\ell}}}, K(X_N)}_n (x) \\
    &= \frac{1}{\sqrt{N^d \lambda_{\ell}}} \sum_{\p \in [N]^d} K(x,x_{\p}) e^{j \frac{2\pi \ell \cdot \p}{N}} \\
    &= \frac{1}{\sqrt{N^d \lambda_{\ell}}} \sum_{\p \in [N]^d} \sum_{\m \in \Integer^d} G[\m] e^{j\m \cdot x} e^{-j \frac{2\pi \m \cdot \p}{N}} e^{j \frac{2\pi \ell \cdot \p}{N}} \\
    &= \frac{1}{\sqrt{N^d \lambda_{\ell}}} \sum_{\m \in \Integer^d} G[\m] e^{j\m \cdot x} \sum_{n=1}^N  e^{-j \frac{2\pi (\m-\ell) \cdot \p}{N}} \\
    &= \frac{N^d}{\sqrt{N^d \lambda_{\ell}}} \sum_{\m \in \Integer^d} G[\m] e^{j\m \cdot x} \mathbbm{1}\{\m - \ell \in N \cdot \Integer\} \\
    \implies \psi_{\ell}(x) &= \sqrt{\frac{N^d}{\lambda_{\ell}}} \sum_{\m \in \Integer} G[\m N + \ell] e^{j (\m N + \ell) \cdot x}
\end{align}
\end{proof}


\begin{lemma}
\label{lem:psi_orthonormal_highd}
The eigenfunctions $\psi_\ell$ (for $\ell \in [N]^d$) are orthogonal in $L^2$ (i.e. $\inner{\psi_\ell, \psi_{k}}_{L^2} = 0$ for $\k \neq \ell$). Let $\lambda_{\ell} = \prod_{i=1}^d \lambda_{\ell_i}$. Further, the eigenfunctions $\psi_\ell$ have norm 
\begin{align}
\|\psi_{\ell}\|_{L^2}^2 = \frac{(2\pi N)^d}{\lambda_\ell} \sum_{m \in \Integer^d} \rbrac{G[\m N + \ell]}^2,\qquad \ell\in[N]^d.    
\end{align}
\end{lemma}
\begin{proof}[Proof of \Cref{lem:psi_orthonormal_highd}]
Suppose $\k \neq \ell$.
\begin{align}
    \inner{\psi_{\ell},\psi_k} &= \sqrt{\frac{N^{2d}}{\lambda_{\ell}\lambda_k}} \sum_{\m,\m^\prime \in \Integer^d} G[\m N + \ell] G[\m^\prime N + \k] \inner{e^{j(\m N + \ell) \cdot x},e^{j(\m N + \k) \cdot x}}_{L^2} \\
    &= 0 
\end{align}
For the second claim,
\begin{align}
\inner{\psi_{\ell}, \psi_{\ell}}_{L^2} &= \frac{N^d}{\lambda_{\ell}} \sum_{\m \in \Integer^d} \rbrac{G[\m N + \ell]}^2 \|e^{j(\m N + \ell) \cdot x}\|_{L^2} \\
&= \frac{(2\pi N)^d}{\lambda_{\ell}} \sum_{\m \in \Integer^d} \rbrac{G[\m N + \ell]}^2
\end{align}
\end{proof}

==> no_arxiv/old/inconsistency_constant.tex <==









% \section{Discussion}

% \paragraph{The Blessing of Dimensionality}
% We can understand how consistency of kernel interpolation is enabled by high dimensions through our results. In particular, the dimension acts as a form of regularization, counter-acting the error due to noise. When the dimensionality is on the scale of the number of samples, the resolution along each dimension will be roughly $N=1$. This is because the total number of samples is $n = N^d (=d)$. Then, by Assumption \ref{assum:coefficient_decay} and the MSE lemma in arbitrary dimension (see Appendix), we have the estimation error is $O(d^{-1}\sigma^2)$. Further, the approximation error does not increase with the number of samples as the inverse bandwidth no longer scales with the number of samples ($M = N \approx 1$ along each dimension). This is in contrast to the fixed dimension case where $M$ must scale with $N$ to make the estimation error vanishing with $N$ (worsening the approximation error). 

% \paragraph{Approximation versus Estimation: a Bias-Variance Tradeoff}



% \section{MSE for General Target Functions}

% We now relax the assumption that the target function is in the span of the represeneters for the data. In particular, where $P_{\X}$ is the $L^2$-projection operator onto the span of the representers and $f^*_{\perp}$ is the component of $f^*$ perpendicular to the span, we can decompose the target function as
% \begin{align}
%     f^*(x) &= P_{\X}(f)(x) + f^*_{\perp}(x) \\
%     &= \sum_{n=1}^N \alpha^*_i k(x,x_i) + f^*_{\perp}(x) \\
%     &= \inner{\alphavec^*,K(X_N,x)}_i + f^*_{\perp}(x)
% \end{align}
% for some $\alphavec^*\in\Real^n.$ Now, note that we can decompose the MSE on the population into three error terms - the estimation error (considered in the previous section), pure approximation error, and the kernelized approximation error. Applying the Pythagorean Theorem,
% \begin{align}
%     (2\pi)^d \text{MSE} = \int_\mc X |f^*(t) - \hat{f}(t)|^2 \dif t &= \int_\mc X |f^*(t) - P_{\X}f^*(t) + P_{\X}f^*(t) - \hat{f}(t)|^2 \dif t \\
%     &= \underbrace{\int_\mc X |f^*(t) - P_{\X}f^*(t)|^2}_{\text{Pure Approximation Error}} + \int_\mc X |P_{\X}f^*(t) - \hat{f}(t)|^2
% \end{align}
% This holds because $\inner{f^*-P_{\X} f^*, \wh f-P_{\X} f^*}_{L^2} = 0$ by definition of the $L^2$ projection.
% We now decompose the second term into the two additional error terms. Define $\alphavec^*$ such that $P_{\X}f^*(x) = \sum_{n=1}^N \alphavec^*_i k(x,x_i) = \inner{\alphavec^*,K(X_N,x)}_i$. Then,
% \begin{subequations}
% \begin{align}
%     \Exp{\int_\mc X |P_{\X}f^*(t) - \hat{f}(t)|^2} &= \Exp{\int |P_{\X}f^*(t) - \inner{\K\inv(\y + \xivec),K(X_N,t)}_i|^2} \\
%     &= \Exp{\int |P_{\X}f^*(t) - \inner{\K\inv(\K\alphavec^* + (f^*_{\perp})_i + \xivec ),K(X_N,t)}_i|^2} \\
%     &= \Exp{\int |P_{\X}f^*(t) - P_{\X}f^*(t)  + \inner{\K\inv((f^*_{\perp})_i + \xi),K(X_N,t)}_i|^2} \\
%     &= \Exp{\int \rbrac{\inner{\K\inv(f^*_{\perp})_i,K(X_N,t)}_i + \inner{\K\inv\xi,K(X_N,t)}_i}^2} \\
%     % &= \int \rbrac{\inner{\K\inv(f^*_{\perp})_i,K(X_N,t)}_i}^2 + \Exp{\int \inner{\K\inv\xi,K(X_N,t)}_i \inner{\K\inv(f^*_{\perp})_i,K(X_N,t)}_i} + \Exp{\int \rbrac{\inner{\K\inv\xi,K(X_N,t)}_i}^2} \\
%     &= \int \rbrac{\inner{\K\inv(f^*_{\perp})_i,K(X_N,t)}_i}^2 + \Exp{\int \rbrac{\inner{\K\inv\xi,K(X_N,t)}_i}^2}
% \end{align}
% \end{subequations}
% where the cross term cancels out since the noise is centered. Finally,
% \begin{align}
%     (2\pi)^d \Exp_\xi{\sbrac{\text{MSE}}} &= \underbrace{\int_\mc X |f^*(t) - P_{\X}f^*(t)|^2}_{\text{Pure Apx. Error}} + \underbrace{\int \rbrac{\inner{\K\inv(f^*(t) - P_{\X}f^*(t))_i,K(X_N,t)}_i}^2}_{\text{Kernelized Apx. Error}} + \underbrace{\Exp{\int \rbrac{\inner{\K\inv\xi,K(X_N,t)}_i}^2}}_{\text{Estimation Error}}
% \end{align}

%\begin{definition}[Kernel Operator]
%Let $\phi_k$ for $\k \in \Integer$ be the eigenfunctions for the two-dimensional kernel operator $T^{\Phi}$ defined as:
%\begin{align}
%    T_{\Phi}[f](x) = \int_{0}^{2\pi} \Phi(x,z) f(z) \dif z 
%\end{align}
%i.e. there exists a sequence $\lambda_k > 0$ for $k \in \Integer$ such that, 
%\begin{align}
%    T_{\Phi}[\phi_k] = \lambda_k \phi_k \quad \forall k \in \Integer_{\geq 0}
%\end{align}
%\end{definition}



==> no_arxiv/old/intro_signal_proc.tex <==
\section{Introduction}

We are interested in studying RKHS estimators with minimal reliance on variational formulations.
\begin{align}
    \wh{y}(x) = \sum_{i=1}^n \alpha(x_i) K(x, x_i) \tag{KR: Kernel Regressor}\\
    \wh{y}(x) = \sum_{i=1}^n y(x_i) K(x,x_i)\tag{KS: Kernel Smoother}
\end{align}

\begin{proposition}
If $\mc H$ is an RKHS then for any monotone function $\phi$,
\begin{align*}
    \argmin{f\in \mc H}\ \sum_{i=1}^n (y_i-f(x_i)) + \lambda\phi(\norm{f}_{\mc H})^2 = \sum_{i=1}^n \alpha(x_i) K(x_i, \cdot)
\end{align*}
furthermore, $\alpha$ satisfies
\begin{align*}
    \sum_{i=1}^n\alpha(x_i) K(x_j, x_i) \left(1+\lambda\phi\left(\sum_{i,j}\alpha(x_i)\alpha(x_j)K(x_i, x_j)\right)\right) = y(x_j)
\end{align*}
\end{proposition}

\section{Signal Reconstruction in 1 dimensions}

Let us start by setting up some notation.
Suppose $y(t)$ is a periodic signal over $t\in\Real$, with period $P$ (s). For a sampling rate $1/T$ (Hz) denote where is the discrete delta function. 


Suppose $y^{(1)}(t) = \cos(2\pi f_0 t)$ for $f_0 > 1/T$, the sampling frequency. Then 
\begin{align*}
Y^{(1)}_T(\omega) &= \sum_{n\in\mathbb{Z}} 
\end{align*}



\begin{theorem}[Shannon-Nyquist theorem]
If $y(t)$ is observed uniformly over the grid $\{i/n\}_{i=1}^n$, then the reconstruction
\begin{align*}
    y(t) = \sum_{i=1}^n y(\frac{i}{n})\cdot \sinc(nt-i)
\end{align*}
achieves $0$ error for band-limited functions $y.$
\end{theorem}


==> no_arxiv/old/notation.tex <==
\appendices
\section{Signal Processing Notation}
\begin{align}
    y(t+P) & = y(t) \tag{Periodic signal},\qquad &t\in\Real\\
    \wb{\delta}(t) &=\mathbf{1}_{\{t=0\}} \tag{Discrete delta}\\
    y_T[n] & = y(nT)\wb{\delta}(t-nT),\qquad &n\in\mathbb{Z} \tag{Sampling}\\
    \text{rect}\left(\frac{t}{P}\right) &= \begin{cases}
    1 & -\frac{P}2\leq t < \frac{P}2\\
    0 & \text{o.w.}
    \end{cases} \tag{Rectangle waveform}\\
    \wb{y}(t) &= y(t)\cdot \text{rect}(t/P)\tag{Truncation}\\
    \wb{y}_T[n] &= y(nT)\wb{\delta}(t-nT) & n\in\mathbb{Z}\cap\left[\tfrac{-P}{2T},\tfrac{P}{2T}\right)\nonumber\\
    Y_T(\omega) &:= \sum_{n\in\mathbb{Z}} y_T[n] e^{-j\omega n} & \omega\in[-\pi,\pi) \tag{DTFT}\\
    \wb{Y}_T(\omega) &:= \sum_{n\in\mathbb{Z}} \wb{y}_T[n] e^{-j\omega n} & \omega\in[-\pi,\pi) \\
    Y(f) &:= \int y(t) e^{-j2\pi ft}dt &f\in\Real\tag{FT}
\end{align}


==> no_arxiv/old/technical_lemmas.tex <==
\section{Technical Lemmas}
\begin{lemma}\label{lem:sum:i} 
For $\theta_i,\theta_j\in\Omega_n$, integers $k\geq 0$, $0\leq \ell\leq \frac{n}{2}$, and $\theta\in\Omega$, we have
\begin{align*}
    \sum_{i=0}^{n-1}
    \cos(\ell(\theta_i-\theta_j))   
    \cos(k(\theta-\theta_i)) 
    =
    n
    \begin{cases}
    \cos(k\theta) & r_n(k)=0\\
    \cos(k(\theta-\theta_j)) & r_n(k)=\frac{n}2\\
    \frac12\cos(k(\theta-\theta_j)) & r_n(k)=\ell\notin\{0,\frac{n}2\}\\
    0 & {\rm otherwise}
    \end{cases}
\end{align*}
\end{lemma}
\begin{proof}
We start by stating the following fact,
for an integer $m\geq 0$, we have 
\begin{align}
\sum_{i=0}^{n-1} \cos(m\theta_i+\phi)=n\cos(\phi)\mathbf{1}_{\{r_n(m)=0\}}.    
\end{align}
Observe that,
\begin{align}
    \sum_{i=0}^{n-1}\cos(\ell(\theta_i-\theta_j))   \cos(k(\theta-\theta_i)) 
    &= \frac12
    \sum_{i=0}^{n-1}
    \cos(\ell(\theta_i-\theta_j)+k(\theta-\theta_i))+   \cos(\ell(\theta_i-\theta_j)-k(\theta-\theta_i))\\
    &=\frac{n}2
    \begin{cases}
    2\cos(k\theta) & r_n(k)=\ell=0\\
    \cos(k\theta-\ell\theta_j) & r_n(k)=\ell\\
    \cos(k\theta+\ell\theta_j) & r_n(k)=-\ell\\
    \cos(k\theta-\frac{n}{2}\theta_j)+\cos(k\theta+\frac{n}{2}\theta_j) & r_n(k) = \frac{n}2\\
    0 & \text{otherwise}
    \end{cases}
\end{align}
 Next,
notice that for $k=mn+\ell$,  we have $k\theta-\ell\theta_j = k(\theta-\theta_j)+(k-\ell)\theta_j= k(\theta-\theta_j)+2\pi mj$. The result follows from the periodicity of cosine. A similar argument holds for the other case of $k=mn-\ell$.
% For the sake of completeness, suppose $n$ is even and $k=(m+\frac12)n$ for some $m$. In that case $\ell=\frac{n}{2}$ is also a valid term and the result holds true for $r_n(k)=\frac{n}{2}$. 
\end{proof}

==> no_arxiv/old/unit_circle.tex <==
\section{Interpolation on Lattices on the Unit circle}
\label{sec:unit_circle}
Let the domain $\Omega:=[-\pi,\pi)$ be the unit circle. And let the observed samples be at $\Omega_n:=\{\theta_i := \frac{2\pi i}{n}  \mid i\in\{0,2,\ldots, n-1\}\}$ for which we observe labels $y_i$. For a kernel $K:\Omega\times \Omega\rightarrow \Real$, let $\Kmat=(K(\theta_i,\theta_j)) \in \Real^{n\times n}$ denote the kernel matrix. For $k\in\Natural,$ denote by $r_n(k) \in (-\frac{n}2,\frac{n}2]$ the integer remainder of $k$ when divided by $n$. Let $h=\frac1M$ be the Kernel width for some integer $M$.

Let $\beta,\beta^M:\Integer\rightarrow\Complex$ and 
\begin{align}
    g(\theta \mod \Omega) &= \sum_{k\in\Integer} \beta[k] \exp(jk\theta)\\
    g(M(\theta \mod \Omega)) &= \sum_{k\in\Integer} \beta^{M}[k] \exp(jk\theta)\\
    \beta^M[k] &= \int_{-\pi}^\pi g(M\theta)\exp(-jk\theta)\dif\theta = \int_{-M\pi}^{M\pi} g(u)\exp(-j(k/M)u)\dif u\\
    &= \wh{g}(\tfrac{k}{M}) - \int_{M\pi}^\infty g(u)\exp(-j\frac{k}{M} u)\dif u - \int_{-\infty}^{-M\pi} g(u)\exp(-j\frac{k}{M} u)\dif u.
\end{align}
We may at a later time use the fact that $g$ is an even function.
% For simplicity, we will assume $n$ is odd.
% \begin{lemma}
% For $\theta,\theta'\in \Omega$, if $K_M(\theta,\theta')=g(M(\theta-\theta') \mod 2\pi)$, for some even function $g:\Omega\rightarrow \Real_+$, then 
% \begin{enumerate}
%     \item $K(\theta,\theta') =\displaystyle \sum_{k\geq 0} c_k \cos({k}(\theta-\theta'))$ where $c_k$ are Fourier series coefficients of $g$, where $\theta,\theta'\in\Omega$.
%     \item $\Kmat$ is a symmetric positive definite Toeplitz structured matrix. 
%     \item $\Kmat_{ij} =\displaystyle \sum_{\ell \leq \frac{n}2} C_\ell \cos(\frac{2\pi}{n}\ell(i-j))$ where $C_\ell = \begin{cases}
%     \displaystyle \sum_{m\geq 0} c_{mn+\ell}+ c_{(m+1)n-\ell} & \ell\notin \{0,\frac{n}{2}\}\\
%     % - \mathbf{1}_{\{n\text{\ \rm is\ even}\}}c_{mn+\frac{n}2}(-1)^{i-j} 
%     \displaystyle\sum_{m\geq 0} c_{mn} & \ell=0\\
%     \displaystyle\sum_{m\geq 0}c_{(m+\frac{1}{2})n} & \ell = \frac{n}{2}\ \text{(only if $n$ is even)}
%     \end{cases}$
%     % , where $\theta_i,\theta_j\in\Omega_n$
%     \item $\displaystyle\Kmat\inv_{ij} = {\frac{1}{n}}\sum_{\ell\leq \frac{n}2} \frac1{C_\ell} \cos(\frac{2\pi}{n}\ell(i-j))$
%     \item\label{lem:existence} Let $\wh y_{int}(\cdot)$ be the interpolator using the kernel $K$. There exists a kernel $\wt K$, such $\wh y_{int}$ is given by the Nadaraya-Watson estimator using $\wt K$, \ie,
%     \begin{align*}
%         \wh y_{int}(\theta)=\sum_{\theta_i \in\Omega_n} y(\theta_i)\wt K(\theta,\theta_i)
%     \end{align*}
%     Furthermore, $\wt K(\theta, \theta') = h(\theta-\theta'\mod 2\pi)$ where $h$ has Fourier series coefficients given by
%     \begin{align*}
%     \wt{c}_k = 
%     \frac{c_k}{C_{|r_n(k)|}}\cdot\begin{cases}
%          1 & r_n(k)\in\{0,\frac{n}2\}\\
%         \frac12 & \text{otherwise}
%     \end{cases}
% \end{align*}
% \end{enumerate}
% \end{lemma}

\begin{lemma}
\label{lemma:kernel_unit_circle}
For $\theta,\theta'\in \Omega$, if $K^M(\theta,\theta')=g(M(\theta-\theta' \mod \Omega))$, for some even function $g:\Real\rightarrow \Real_+$, then 
\begin{enumerate}
    \item $K^M(\theta,\theta') =\displaystyle \sum_{k\in\Integer} \beta^M[k] 
    \exp(j{k}(\theta-\theta'))$, where $\theta,\theta'\in\Omega$.
    \item $\Kmat$ is a symmetric positive definite Toeplitz matrix with
    \begin{align}
        \Kmat = \sum_{\ell\in[n]} \gamma^M[\ell]\v_\ell\v_\ell\herm
    \end{align}
    where $\v_\ell=\begin{bmatrix}1 & \exp(j\tfrac{2\pi}{n}\ell) & \exp(j\tfrac{2\pi}{n}2\ell) & \ldots & \exp(j\tfrac{2\pi}{n}(n-1)\ell)\end{bmatrix}\T$,
    where
    \begin{align}
        \gamma^M[\ell] = \sum_{m\in\Integer}\beta^M[mn+\ell]
    \end{align}
    \item The inverse satisfies,
    \begin{align}
        \Kmat\inv = \frac1n\sum_{\ell\in[n]} \frac1{\gamma^M[\ell]}\v_\ell\v_\ell\herm
    \end{align}
    % \item $\Kmat_{ij} =\displaystyle \sum_{\ell \leq \frac{n}2} C_\ell \cos(\frac{2\pi}{n}\ell(i-j))$ where $C_\ell = \begin{cases}
    % \displaystyle \sum_{m\geq 0} c_{mn+\ell}+ c_{(m+1)n-\ell} & \ell\notin \{0,\frac{n}{2}\}\\
    % % - \mathbf{1}_{\{n\text{\ \rm is\ even}\}}c_{mn+\frac{n}2}(-1)^{i-j} 
    % \displaystyle\sum_{m\geq 0} c_{mn} & \ell=0\\
    % \displaystyle\sum_{m\geq 0}c_{(m+\frac{1}{2})n} & \ell = \frac{n}{2}\ \text{(only if $n$ is even)}
    % \end{cases}$
    % , where $\theta_i,\theta_j\in\Omega_n$
    % \item $\displaystyle\Kmat\inv_{ij} = {\frac{1}{n}}\sum_{\ell\leq \frac{n}2} \frac1{C_\ell} \cos(\frac{2\pi}{n}\ell(i-j))$
    \item\label{lem:existence} Let $\wh y_{int}(\cdot)$ be the interpolator using the kernel $K^M$. There exists a kernel $\wt K^M_n$, such $\wh y_{int}$ is given by,
    \begin{align*}
        \wh y_{int}(\theta)=\frac1n\sum_{\theta_i \in\Omega_n} y(\theta_i)\wt K^M_n(\theta,\theta_i)
    \end{align*}
    Furthermore, $\wt K^M_n(\theta, \theta') = \wt g_n(M(\theta-\theta')\mod \Omega)$ where $\wt g_n$ has Fourier expansion
    \begin{align*}
    \wt g_n(M\theta \mod \Omega) &= \sum_{k\in\Integer} \wt\beta_n^M[k]\exp(jk\theta)\\
    \wt{\beta}^M_n[k] &= 
    \frac{\beta^M[k]}{\gamma^M[r_n(k)]}=
    % \begin{cases}
    % \frac{\beta[k/M]}{\gamma^M[r_n(k)]} & r_M(k)=0\\
    % 0 & \text{\rm otherwise}
    % \end{cases}
    \\
    \wt{\beta}_n[k] &= 
    \frac{\beta[k]}{\gamma^1[r_n(k)]}
\end{align*}
\end{enumerate}
\end{lemma}


% $$\sum_{0\leq \ell<n/2} C_\ell \cos(2\pi \ell i/n)\cos(2\pi\ell j/n)+\sum_{n/2\leq \ell< n} C_\ell\sin(2\pi\ell i/n)\sin(2\pi\ell j/n)$$

% $$[\cos(2\pi \ell i/n)]_i,\qquad [\sin(2\pi \ell i/n)]_i$$

% $$A\x_i = \lambda_i\x_i$$

% $$A\X=\X\Lambda$$

% $$A=\X\Lambda\X\T \implies A\inv= \X \Lambda\inv\X\T$$

% $$a_{ij} = \sum_{\ell=1}^n \lambda_\ell x_{\ell i}x_{\ell j}$$

% $$\lambda_\ell=C_\ell,\qquad x_{i\ell}=\cos(2\pi\ell i/n) \ \ell<n/2,\qquad \sin(2\pi\ell i/n)\ \ell > n/2$$
% \begin{proof}[Proof of Part \ref{lem:existence}]
% In what follows, $i,j,k,\ell$ are all integers, with bounds $0\leq i,j\leq n-1$, $0\leq \ell\leq  n/2 $ and $k\geq 0$. 
% The kernel interpolator for an arbitrary $\theta\in\Omega$ and $\theta_i,\theta_j\in\Omega_n$ is given by
% \begin{align}
%     \wh y(\theta) 
%     &= \sum_{i} \alpha_i K(\theta,   \theta_i)
%     = \sum_{i}\left( \sum_{j}\Kmat\inv_{ij} y_j \right)g(\theta-\theta_i)\\
%     &= {\frac1n}\sum_{j} y_j \sum_{i} \sum_{\ell} \frac1{C_\ell} \cos(\ell(\theta_i-\theta_j))  \sum_{k}c_k \cos(k(\theta-\theta_i))\\
%     &= {\frac1n}\sum_{j} y_j  \sum_{\ell}\sum_{k} \frac{c_k}{C_\ell} \sum_{i}\cos(\ell(\theta_i-\theta_j))   \cos(k(\theta-\theta_i))\\
%     &\overset{\rm (a)}=\sum_{j}y_j \sum_{\ell} \sum_{|r_n(k)|=\ell} \frac{c_k}{2C_\ell}(1+\mathbf{1}{\{r_n(k)\in\{0,\frac{n}2\}\}})\cos(k(\theta-\theta_j))\\
%     &=\sum_{j}y_j \sum_{k}  \frac{c_k}{2C_{|r_n(k)|}}(1+\mathbf{1}{\{r_n(k)\in\{0,\frac{n}2\}\}})\cos(k(\theta-\theta_j))=\sum_j y_j h(\theta-\theta_j)
% \end{align}
% where (a) follows from \Cref{lem:sum:i}. In the last equality above we introduce $h$, an even function with Fourier series coefficients
% \begin{align*}
%     \wt{c}_k:=\frac{c_k}{C_{|r_n(k)|}}\cdot\begin{cases}
%     1 & r_n(k)\in\{0,\frac{n}2\}\\
%     \frac12 & \text{otherwise}\\
%     \end{cases}
% \end{align*}
% \end{proof}

\subsection{Lower bound on \texorpdfstring{$L^2$}{L2} error for bandlimited functions}
Let $y^*:\Omega\rightarrow\Complex$ be a bandlimited function with bandwidth $B,$ and $Y^*:\Integer\rightarrow\Complex$ be its fourier series \ie,
\begin{align*}
    y^*(\theta) = \sum_{\substack{k\in\Integer\\{|k|\leq B/2}}} Y^*[k]\exp(jk\theta)
\end{align*}
We note the following identity for ${n>B}$,
\begin{align*}
    y^*(\theta) &= \frac1n\sum_{i=1}^n y^*(\theta_i)h(\theta-\theta_i)\\
    h(\theta)&:= \sum_{ \abs{k}\leq{B}/2} \exp(jk\theta)
\end{align*}
Now consider the $L^2$ error in the noiseless case where the labels are given by $y_i=y^*(\theta_i),$ 
\begin{align}
    \norm{y^*-\wh y}_{L^2(\Omega)}^2
    &=\int |y^*(\theta)-\wh y(\theta)|^2 \dif \theta \\
    &=\int \left|\frac1n\sum_{i=1}^n y^*(\theta_i)\cbrac{h(\theta-\theta_i)- \wt{g}_n(M(\theta-\theta_i)\mod\Omega)}\right|^2 \dif \theta\\
    % &=\int \left|\frac1n\sum_{i=1}^n y^*(\theta_i) e^M_n(\theta-\theta_i)\right|^2 \dif \theta\\
    % &\overset{\red{?}}\geq \int\left|\int y^*(u)e^M_n(\theta-u) \dif u\right|^2\dif\theta\\
    &= \sum_{k} |Y^*[k]|^2|E^M_n[k]|^2\\
    &= \sum_{|k|<\frac{B}2} |Y^*[k]|^2|E^M_n[k]|^2
\end{align}
where %$e^M_n(\theta) := \sinc(\frac{n}2\theta)-\wt g_n(M\theta\mod\Omega)$ and
$E_n^M[k]=\mathbf{1}{\{|k|\leq\frac{B}2\}}-\wt\beta^M_n[k]$ is the Fourier series of expansion of $h(\theta)- \wt{g}_n(M\theta\mod\Omega)$.

% \subsection{Analysis of equivalent Kernel}
% Next, suppose $n$ is odd for simplicity and $c_k = e^{-ak},$ for some positive \red{bandwidth parameter} $a$, then
% \begin{align}
%     C_\ell &= 
%     \frac1{1-e^{-an}}\cdot \begin{cases}
%     1 & \ell = 0\\
%     e^{-a\ell}+e^{-a(n-\ell)} & \ell \notin \{0,\frac{n}2\}\\
%     e^{-an/2} & \ell = \frac{n}2
%     \end{cases}\\
%     \wt c_{mn+\ell} &= \frac{e^{-amn}(1-e^{-an})}{1+e^{-a(n-2\ell)}}
% \end{align}

% \paragraph{Next:}
% \begin{enumerate}
%     \item We know bias of NWE interpolator grows with its kernel-width parameter
%     \item We need to relate a kernel width parameter for $K$ or $g$ to $h$ or $\wt K$
%     \item This (\red{hopefully}) shows a lower bound on bias in terms of kernel width of $K$.
% \end{enumerate}






==> no_arxiv/old/upper_bounds.tex <==
\section{Upper Bounding Generalization Error}
We seek the maximal MSE that can occur for a function $f = \sum_k v_k \phi_k$ on the unit circle for fixed bandwidth parameters $M^{-1}$. By lemma \ref{lemma:MSE_1d}, we have an exact expression for the MSE that is a quadratic function of the $v_k$ variables. We restrict the set of functions we consider to those with $H$-norm bounded by $1$ for the RKHS corresponding to $M=1$. 

We can then formulate this problem as a quadratic optimization:
\begin{align}
    \max{\v} \frac{1}{2\pi} \rbrac{\sum_{k} v_k^2 - \sum_{\ell=0}^{N-1} \frac{R_{\ell}^2}{r_{\ell}}} + \frac{1}{2\pi} \sum_{\ell = 0}^{N-1} \rbrac{\frac{\beta_{\ell}}{\gamma_{\ell}} - \frac{R_{\ell}}{r_{\ell}}}^2 r_{\ell} - \lambda \rbrac{\sum_{k} \frac{v_k^2}{G^1[k]} - 1}
\end{align}
We will show we can formulate this as a generalized eigenvalue problem. This optimization is equivalent to the following:
\begin{align}
    &\max{\v} \v^{\tran}\v - \sum_{\ell=0}^{N-1} \frac{(G_{M,\ell}^{\tran}\v)^2}{r_{\ell}} + \sum_{\ell = 0}^{N-1} \rbrac{\frac{\v^{\tran}\mathbbm{1}_{\ell}}{\gamma_{\ell}} - \frac{G_{M,\ell}^{\tran}\v }{r_{\ell}}}^2 r_{\ell} -  2\pi \lambda \rbrac{\G\inv \v^{\tran}\v - 1} \\
    &= \max{\v} \v^{\tran}\v - \sum_{\ell=0}^{N-1} \frac{\v^{\tran}G_{M,\ell}G_{M,\ell}^{\tran}\v}{r_{\ell}} + \sum_{\ell = 0}^{N-1} \rbrac{\frac{\v^{\tran}\mathbbm{1}_{\ell}\mathbbm{1}_{\ell}^{\tran}\v}{\gamma^2_{\ell}} - \frac{\v^{\tran}(\mathbbm{1}_{\ell}G_{M,\ell}^{\tran} + G_{M,\ell}\mathbbm{1}_{\ell}^{\tran})\v}{\gamma_{\ell}r_{\ell}} + \frac{\v^{\tran}G_{M,\ell}G_{M,\ell}^{\tran}\v }{r^2_{\ell}}} r_{\ell}\\
    &-  2\pi \lambda \rbrac{\G\inv \v^{\tran}\v - 1} \\
    &= \max{\v} \v^{\tran}\rbrac{I - \sum_{\ell=0}^{N-1} \frac{G_{M,\ell}G_{M,\ell}^{\tran}}{r_{\ell}} + \sum_{\ell = 0}^{N-1} \rbrac{\frac{\mathbbm{1}_{\ell}\mathbbm{1}_{\ell}^{\tran}r_{\ell}}{\gamma^2_{\ell}} - \frac{\mathbbm{1}_{\ell}G_{M,\ell}^{\tran} + G_{M,\ell}\mathbbm{1}_{\ell}^{\tran}}{\gamma_{\ell}} + \frac{G_{M,\ell}G_{M,\ell}^{\tran} }{r_{\ell}}} -  2\pi \lambda \G\inv }\v  + 2\pi \lambda \\
    &= \max{\v} \v^{\tran}\rbrac{\underbrace{I + \sum_{\ell = 0}^{N-1} \rbrac{\frac{\mathbbm{1}_{\ell}\mathbbm{1}_{\ell}^{\tran}r_{\ell}}{\gamma^2_{\ell}} - \frac{\mathbbm{1}_{\ell}G_{M,\ell}^{\tran} + G_{M,\ell}\mathbbm{1}_{\ell}^{\tran}}{\gamma_{\ell}}}}_{\A} -  2\pi \lambda \G\inv }\v  + 2\pi \lambda \\
    &= \max{\v} \v^{\tran}\rbrac{\A -  2\pi \lambda \G\inv }\v  + 2\pi \lambda
\end{align}
Setting the derivatives to $0$ of $v_k$, we derive the generalized eigenvalue equation. In particular we seek the maximum eigenvalue $\lambda$ such that:
\begin{align}
    \A\v &= 2\pi \lambda \G\inv \v \\
    \iff \frac{1}{2\pi}\G\A\v &= \lambda \v 
\end{align}
Therefore, we seek the maximum (standard) eigenvalue of the matrix $\frac{1}{2\pi}\G\A$. Let $h^M_{\ell} = \frac{(G_{M,\ell})^{\tran} (G_{M,\ell})}{(G_{M,\ell})^{\tran} \mathbbm{1}_{\ell}} = \frac{r_{\ell}}{\gamma_{\ell}}$.
\begin{align}
    \G\A &= \G + \sum_{\ell=0}^{N-1} \rbrac{\frac{\G\mathbbm{1}_{\ell}\mathbbm{1}_{\ell}^{\tran}r_{\ell}}{\gamma^2_{\ell}} - \frac{\G(\mathbbm{1}_{\ell}G_{M,\ell}^{\tran} + G_{M,\ell}\mathbbm{1}_{\ell}^{\tran})}{\gamma_{\ell}}} \\
    &= \G + \sum_{\ell=0}^{N-1} \rbrac{\frac{G_{\ell}\mathbbm{1}_{\ell}^{\tran} h^M_{\ell}}{(G_{M,\ell})^{\tran} \mathbbm{1}_{\ell}} - \frac{\G(\mathbbm{1}_{\ell}G_{M,\ell}^{\tran} + G_{M,\ell}\mathbbm{1}_{\ell}^{\tran})}{(G_{M,\ell})^{\tran} \mathbbm{1}_{\ell}}}
\end{align}
We can upper bound the maximum eigenvalue of this matrix by its trace.
\begin{align}
    \trace(\G\A) &= \sum_{k \in \Integer} G[k] + \sum_{\ell=0}^{N-1} \gamma_{\ell}^{-1} \rbrac{h^M_{\ell} \trace(G_{\ell}\mathbbm{1}_{\ell}^{\tran})  - \trace(\G\mathbbm{1}_{\ell}G_{M,\ell}^{\tran}) - \trace(\G G_{M,\ell}\mathbbm{1}_{\ell}^{\tran})} \\
    &= \sum_{k \in \Integer} G[k] + \sum_{\ell=0}^{N-1} \gamma_{\ell}^{-1} \rbrac{h^M_{\ell} \trace(\mathbbm{1}_{\ell}^{\tran} G_{\ell})  - \trace(G_{M,\ell}^{\tran}G_{\ell}) - \trace(G_{M,\ell}^{\tran}G_{\ell})} \\
    &= \sum_{k \in \Integer} G[k] + \sum_{\ell=0}^{N-1} \gamma_{\ell}^{-1} \rbrac{h^M_{\ell} \mathbbm{1}_{\ell}^{\tran} G_{\ell}  - 2G_{M,\ell}^{\tran}G_{\ell}} 
\end{align}

\begin{theorem}
When $M \leq N$, kernel interpolation is inconsistent for all functions on the unit circle in the given noise model. When $M \geq N^2$ there exists functions for which kernel interpolation is inconsistent and for which it is consistent. Further, the set of these functions contracts monotonically as $M$ increases. 
\end{theorem}
\begin{proof}
For the lower bounds in this section we use the trivial constant function $f = \sqrt{G[1]}$. This is equivalent to setting $v_1 = \sqrt{G[1]}$ and all other $v_k$ to $0$. We then show the bound from this example is tight. 

\underline{Case 1. $M \leq N$}

For the upper bound, we use the trace of $\G\A$. For the given N,
\begin{align}
    \trace(\G\A) &= \sum_{k \in \Integer} G[k] + \sum_{\ell=0}^{N-1} \frac{1}{\mathbbm{1}_{\ell}^{\tran} G_{\ell}} \rbrac{G_{\ell}^{\tran}G_{\ell} - 2G_{\ell}^{\tran}G_{\ell}} \\
    &= \sum_{\ell=0}^{N-1} \rbrac{ G_{\ell}^{\tran}\mathbbm{1}_{\ell} - \frac{G_{\ell}^{\tran}G_{\ell}}{\mathbbm{1}_{\ell}^{\tran} G_{\ell}}}
\end{align}
For all the kernels we consider $\sum_{|k| \geq 1} G[k] = O(G_0)$. Therefore, the maximum eigenvalue is at most a small constant times $G_0$, and we can simplify the MSE bound to,
\begin{align}
    \text{MSE} \leq O(G_0) + (1 - o(1))\sigma^2 N
\end{align}
where the noise term approaches $\sigma^2$ with $N \rightarrow \infty$. For the lower bound, we use $v_0 = G[0]^{1/2}$ and all other $v_k=0$. Then, the MSE is at least the first and third terms:
\begin{align}
    \text{MSE} &\geq \frac{1}{2\pi}(G_0 - \frac{G_0^3}{4G_0^2}) + (1-o(1))\sigma^2 N\\
    &= \frac{3}{8\pi}G_0 + (1-o(1))\sigma^2 N
\end{align}

Although we provide a specific lower bound that is strictly greater than the noise level (by a factor of $G_0$), any kernel on data from a target function $f_0$ will be inconsistent (as the noise term is independent of the function). In particular, the error will grow with the number of samples. 

\underline{Case 2. $M\geq N^2$}

In this case, using the same adversarial example, we can lower bound the MSE by (for some constants $C_1,C_2,C_3>0$):
\begin{align}
    \text{MSE} &\geq \frac{1}{2\pi}(G_0 - \frac{C_1 G_0^2}{N}) + \frac{1}{2\pi}(\frac{C_2}{N} - \frac{C_3}{N})^2 N + \frac{\sigma^2N^2}{M} \\
    &\geq \frac{G_0}{2\pi} + O(1/N) + \frac{\sigma^2N^2}{M}
\end{align}
For $M \gg N^2$, this approaches $\frac{1}{2\pi}G_0$. Recall that the MSE is the sum of two approximation error terms and an estimation error. This approximation error characterizes how far the target function is from the span of the representers of the given banwidth ($1/M$). Therefore, in the regime $M \geq N^2$, there exist functions for which kernel interpolation is consistent - namely those that are well approximated by the span of the representers.  

For the upperbound, we again have:
\begin{align}
    \text{MSE} \leq \frac{\sigma^2N^2}{M} + \trace(GA) \leq \sum_{k \in \Integer} G[k] + O(1/N) + \frac{\sigma^2N^2}{M}
\end{align}

\end{proof}

==> sections/all_kernels.tex <==
\subsection{Proof of Theorem \ref{theorem:inconsistent_all_kernel}}

We construct a target function $f^* = \sum_{k\in\Integer}V[k]\phi_k$ that is inconsistent for all kernels. For a given sample size $N$ and kernel $K$ with Fourier series $G,$ define the map $A_N:[N]\rightarrow \Integer$, given by
\begin{align}
    A_N(i) = 
    \begin{cases}
    0 & \text{if } \frac{\norm{G_i}}{\norm{G_i}_1} = \Omega(1)\\
    & \text{if } \frac{\norm{G_i}}{\norm{G_i}_1} = o(1)\\
    \end{cases}
\end{align}

Suppose $V[A(i)m + i] = \frac{1}{\sqrt{N}}$ for $i \in [N]$ and a map $A:[N] \rightarrow \Integer$ to be chosen later. Then $\|V\| = 1$, and the function is continuous for derivatives of all orders. 

From Lemma \ref{lem:MSE_1d}, we have
\begin{align}
    \mc E^\apx + \mc E^\noisy
    &\geq \frac{1}{N} \sum_{i=0}^{N-1} \rbrac{1 - \frac{G[A(i)N + i]^2}{\norm{G_i}^2}} +  \sigma^2 \round{\frac{\norm{G_i}}{\norm{G_i}_1}}^2
\end{align}

Let $i \in [N]$. If $\|G_i\| = \Omega(\|G_i\|_1)$, then the rightmost term (the contribution from the noisy estimation error) is $\Omega(\sigma^2)$. In this case $A(i) = i$.

Suppose instead, $\|G_i\| = o(\|G_i\|_1)$. In this case, it must be that there are two integers $m,m' \in \Integer$, such that $G[mN + i] = O(G[m'N + i])$. We define the map $A$ from earlier to be $A(i) = m$, and define a similar map $B:[N] \rightarrow \Integer$, such that $B(i) = m'$. In this case,
\begin{align}
    \frac{G[A(i)m + i]^2}{\norm{G_i}^2} &\leq  \frac{G[A(i)m + i]^2}{G[A(i)m + i]^2 + G[B(i)m + i]^2} = O(1) \\
    \implies \rbrac{1 - \frac{G[A(i)m + i]^2}{\norm{G_i}^2}} &= \Omega(1)
\end{align}
This proves the theorem.




